Non determinism through type isomorphism

We define an equivalence relation on propositions and a proof system where equivalent propositions have the same proofs. The system obtained this way resembles several known non-deterministic and algebraic lambda-calculi.

==> eptcsdata.tex <==
\providecommand{\firstpage}{137}
\providecommand{\publicationstatus}{D. Kesner and P. Viana (Eds.): LSFA 2012\\
EPTCS 113, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.113.13}{10.4204/EPTCS.113.13}}

